Conformal Classification with Equalized Coverage for Adaptively Selected Groups

This paper introduces a conformal inference method to evaluate uncertainty in classification by generating prediction sets with valid coverage conditional on adaptively chosen features. These features are carefully selected to reflect potential model limitations or biases. This can be useful to find a practical compromise between efficiency -- by providing informative predictions -- and algorithmic fairness -- by ensuring equalized coverage for the most sensitive groups. We demonstrate the validity and effectiveness of this method on simulated and real data sets.

==> acknolwedgement.tex <==

Software implementing the algorithms and conducting data experiments is accessible online at~\url{https://github.com/FionaZ3696/Adaptively-Fair-Conformal-Prediction.git}.

\subsection*{Acknowledgments}
The authors thank the Center for Advanced Research Computing at the University of Southern California for providing computing resources. The authors also thank Xin Tong for helpful suggestions. Y.~Z.~and M.~S.~were supported by NSF grant DMS 2210637.
